Exploring turnover, retention and growth in an OSS Ecosystem

The Gentoo ecosystem has evolved significantly over 23 years, highlighting the critical impact of developer sentiment on workforce dynamics such as turnover, retention, and growth. While prior research has explored sentiment at the project level, sentiment-driven dynamics at the component level remain underexplored, particularly in their implications for software stability. This study investigates the interplay between developer sentiment and workforce dynamics in Gentoo. The primary objectives are to (1) compare workforce metrics (turnover, retention, and growth rates) between sentiment-positive (SP) and sentiment-negative (SN) components, (2) examine temporal trends across three time phases, and (3) analyze the impact of these dynamics on software stability. A mixed-method approach was employed, integrating sentiment analysis of mailing lists and commit histories using the SentiStrength-SE tool. Workforce metrics were statistically analyzed using Pearson Correlation Matrix and Mann-Whitney U tests. The analysis focused on the most SP and SN components in the ecosystem. SN components exhibited higher retention rates but slower growth and turnover compared to SP components, which showed dynamic contributor behavior but reduced long-term stability. Temporal analysis revealed significant variations in workforce dynamics over three phases, with developer retention correlating positively with modifications in both sentiment groups. Tailored strategies are necessary for managing sentiment-driven dynamics in OSS projects. Improving \textit{adaptability} in SN components, and \textit{continuity} in SP components, could improve project sustainability and innovation. This study contributes to a nuanced understanding of sentiment's role in workforce behavior and software stability within OSS ecosystems.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sections/introduction.tex <==
\section{Introduction}
Open Source Software (OSS) ecosystems rely on the collaborative efforts of distributed developers, where developer engagement, retention and turnover play crucial roles in ensuring long-term project sustainability. Sentiment expressed in developer communications, such as mailing lists and commit messages, reflects not only interpersonal dynamics but also underlying project challenges and successes. Prior research highlights the significance of sentiment analysis in understanding developer behaviors and project outcomes \cite{Guzman2014Sentiment, Ferreira2019Longitudinal}. However, much of this work focuses on project-level analyses, leaving component-level dynamics underexplored.

The Gentoo Linux ecosystem, a large OSS project established in 1999, provides a unique opportunity to study sentiment-driven workforce dynamics. Gentoo’s codebase is organized into categories, which represent components where developers collaborate and contribute. While existing studies have explored developer sentiment in GitHub commit logs \cite{Sinha2016Analyzing} or email threads \cite{Ferreira2019Longitudinal}, these studies often focus on broader, project-level trends. For instance, Guzman et al. \cite{Guzman2014Sentiment} and Sinha et al. \cite{Sinha2016Analyzing} analyzed commit messages to examine emotional patterns, while Ferreira et al. \cite{Ferreira2019Longitudinal} studied email sentiments over shorter time frames. These studies employed single datasets and project-level resolutions, overlooking finer-grained insights at the component level. Additionally, the role of workforce metrics—turnover, retention and growth—remains underexplored in sentiment-affected components.

Behavioural studies in OSS further emphasize the interplay between developer activity and project stability \cite{Robinson2016Developer, Majumder2022Revisiting}. For example, Robinson et al. \cite{Robinson2016Developer} examined sentiment-related behaviours across projects, while Zhou and Mockus \cite{Zhou2012What} identified drivers of sustained contributions. However, these studies fail to account for sentiment-driven dynamics at a granular level, such as specific components within a project. The implications of turnover and retention on component stability and the differences between sentiment-positive and sentiment-negative categories remain unaddressed.

To address these gaps, this study investigates developer dynamics in the Gentoo ecosystem over a 23-year period (2000–2023). We integrate two datasets (mailing list communications and commit histories) to explore three workforce aspects: turnover, retention and growth. Specifically, we aim to analyze the following:
\begin{itemize}
    \item Differences in turnover, retention and growth rates between sentiment-positive and sentiment-negative components.
    \item Temporal trends in workforce dynamics across distinct time periods.
    \item The impact of workforce metrics (e.g., retention and turnover) on the stability and evolution of sentiment-affected components.
\end{itemize}

Unlike previous studies that rely on single datasets or broader project-level analyses, we focus on a deeper, component-level granularity, allowing for a nuanced understanding of sentiment-driven dynamics. This approach provides insights into how developer sentiment influences workforce behavior and software stability at a more localized level, addressing critical gaps in current literature.

%change labels to fit the ones in the paper
The remainder of this paper is organized as follows: Section 2 reviews related work on sentiment analysis and developer dynamics in OSS. Section 3 outlines the data collection, preprocessing and analysis methods. Section 4 presents our findings on workforce metrics and their relationships with sentiment-affected components. Section 5 discusses the broader implications for OSS management, while Section 6 addresses threats to validity. Finally, Section 7 concludes the paper and outlines directions for future research.

